LocalGCL: Local-aware Contrastive Learning for Graphs

Graph representation learning (GRL) makes considerable progress recently, which encodes graphs with topological structures into low-dimensional embeddings. Meanwhile, the time-consuming and costly process of annotating graph labels manually prompts the growth of self-supervised learning (SSL) techniques. As a dominant approach of SSL, Contrastive learning (CL) learns discriminative representations by differentiating between positive and negative samples. However, when applied to graph data, it overemphasizes global patterns while neglecting local structures. To tackle the above issue, we propose \underline{Local}-aware \underline{G}raph \underline{C}ontrastive \underline{L}earning (\textbf{\methnametrim}), a self-supervised learning framework that supplementarily captures local graph information with masking-based modeling compared with vanilla contrastive learning. Extensive experiments validate the superiority of \methname against state-of-the-art methods, demonstrating its promise as a comprehensive graph representation learner.

==> recycle_bin/What_do_CL_and_MM_Learn_from_Graphs.tex <==
\section{What do CL and MM Learn from Graphs}
\label{sec:what}

To explore which aspects of graph information are captured by the CL and MM in graph representation learning, it's crucial to dive deep into their learning processes and training objectives.

The primary goal of CL is to ensure the model can differentiate between positive and negative samples of the graph. In this context, the model accentuates discerning the overarching relationships and patterns within the entire graph or its larger subgraphs. To differentiate between two similar graphs, identifying the global patterns within a graph is usually more pivotal than pinpointing subtle disparities. On the other hand, MM involves randomly obscuring certain sections of the graph and predicting or restoring these sections, necessitating a heightened sensitivity to granular details when processing graph data. Hence, it places more emphasis on nuances and local structures within the graph, like a minor subgraph pattern or the subtle relationships between a node and its neighboring nodes.

% To further validate these observations, we conduct experiments on the IMDB-B dataset using the GraphMAE \cite{hou2022-graphmae} and GraphCL \cite{you2020-graph}. We initially train both models on the same training set, and to ensure the comparability of their parameters, both use GATs with identical parameters as their encoders. In the test set, we fragment the original graphs into several subgraphs and recombine them to form new graphs. These reconstructed graphs exhibit significant global information differences but minimal local discrepancies compared to the original ones. By contrasting their similarities in the embedding space after encoding, we can deduce which aspects of graph information each respective method learns.

To validate our observations on the IMDB-B dataset, we train both GraphMAE \cite{hou2022-graphmae} and GraphCL \cite{you2020-graph} on the same training set. For the test set, we fragment original graphs and recombine them into reconstructed versions with distinct global and minor local differences. By contrasting their similarities in the embedding space after encoding, we can deduce which aspects of graph information each respective method learns.

\begin{figure}[htb]

\begin{minipage}[b]{0.40\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image/cl_before.png}}
  \centerline{(a)}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.40\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image/mm_before.png}}
  \centerline{(b)}\medskip
\end{minipage}
\vspace{0.2cm} % You can adjust this space as needed

\begin{minipage}[b]{0.40\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image/cl_after.png}}
  \centerline{(c)}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.40\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image/mm_after.png}}
  \centerline{(d)}\medskip
\end{minipage}

\caption{Comparison of embeddings from reconstructed graphs and original graphs using GraphCL and GraphMAE. (a, c) show embeddings from GraphCL before and after reconstruction, respectively. (b, d) depict embeddings from GraphMAE before and after reconstruction.The embeddings in GraphMAE show minor changes, maintaining high consistency and emphasizing local information, whereas in GraphCL they undergo significant alterations, suggesting that CL focuses more on global features, whereas MM emphasizes local information.}
\label{fig:vis}

\end{figure}

% We select the embeddings of the reconstructed graphs and original graphs from two classes for comparison, as visualized in Fig.\ref{fig:vis}. As can be seen, after encoding with GraphMAE, the relative distance between the embeddings of the reconstructed graph and the original graph only undergoes minor changes. On the reconstructed graph, the two classes also differentiate distinctly. However, after encoding with GraphCL, the embedding distribution of the reconstructed graph undergoes significant alterations compared to the original graph embedding, with different categories of reconstructed graphs appearing to mix up. These results suggest that GraphMAE primarily focuses on the local information of the graph, maintaining high embedding consistency during graph reconstruction. In contrast, GraphCL leans more towards the global structure of the graph, resulting in significant changes in embedding distribution when there are alterations in the global structure. This further confirms that GraphMAE learns local details, while GraphCL prioritizes capturing global patterns.
We select the embeddings of the reconstructed and original graphs from two classes for comparison, as visualized in Fig.\ref{fig:vis}. After encoding with GraphMAE, the distance between the embeddings of the reconstructed and original graphs experiences minor changes, and the two classes differentiate distinctly on the reconstructed graph. However, with GraphCL, the embedding distribution of the reconstructed graph shows significant alterations, with categories appearing to mix. These results indicate that GraphMAE emphasizes the local information, maintaining consistency during graph reconstruction, while GraphCL focuses on the global structure, leading to notable changes in embedding distribution upon alterations in the global structure.

Given the contrasting focuses of CL on global similarities and differences and MM on restoring local structures, integrating the two presents a challenge for comprehensive graph information extraction. Simultaneously optimizing these opposing objectives can lead to optimization or convergence issues. For instance, while emphasizing global structure, the model might overlook local details and vice versa. This balance between global and local perspectives complicates the integration of the two methods.

==> recycle_bin/preliminary.tex <==
\section{Preliminary}
\label{sec:prelim}
% \subsection{Graph Representation Learning}
% Utilizing graph data directly poses challenges in various machine learning tasks, primarily due to the inadequacy of conventional algorithms in handling the intricate nature of graph structures.
% The emergence of graph representation learning addresses this issue effectively. 
% Graph representation learning aims to encode the structural information, node attributes, or other graph-specific features into low-dimensional vectors, which can then be used by conventional machine learning algorithms.
% This technique masterfully encapsulates the topological structure and inter-node dynamics present in the graph, converting them into fixed-size vector, thereby rendering the graph data more comprehensible and accessible for conventional machine learning models.

% The prowess of graph representation learning stems from its capacity to grasp the intricate structures and inter-nodal relationships inherent in graphs. 
% This capability presents both traditional machine learning and deep learning techniques with a straightforward and efficient way to manage graph data. By crafting meaningful embeddings for entities within the grph, these embeddings do more than just capturing local interconnections; they encapsulate the broader global framework, thus enriching tasks such as classification, clustering, and recommendation with invaluable insights. 
% Additionally, converting the graph's architecture into low-dimensional vectors not only paves the way for processing large-scale graph data but also dramatically reduces storage and computational complexity.

% \subsection{Self-supervised learning}

% Self-supervised learning is a machine learning paradigm that doesn't rely on explicit labeled data. Instead, it uses certain parts of the data as a supervisory signal to train models. This approach allows models to learn useful representations from unlabeled data, providing meaningful features for various downstream tasks. 
% Owing to its intrinsic wealth of structure and attributes, graph data has unique advantages in self-supervised learning within the sphere of graph representation learning. At present, contrastive learning and masking-based modeling reign as the predominant self-supervised techniques in graph representation.

% \textbf{Contrastive learning.} 
% Contrastive learning stands as an unsupervised learning technique whose fundamental principle lies in learning feature representations by comparing the similarities and differences between data points.
% When applied to graph data, the key idea of contrastive learning is to maximize the consistency between two augmented views of a given graph through data augmentation [], training the model to emphasize the representations of the same graph in varied views and diminish similarity with negative samples. 
% This method facilitates capturing global characteristics of graphs, proving invaluable for tasks like graph classification. 
% Given that the essence of contrastive learning revolves around differentiating positive samples of a given graph from its corresponding negative samples, it often places greater emphasis on identifying global patterns in the entire graph or its expansive subgraphs over local changes.
% Hence, the application of contrastive learning on graph data typically places more emphasis on capturing global structures and major subgraph patterns. However, this also unveils its limitation that it might not excel in detecting subtle differences or local patterns within graphs.

% \textbf{Masking-based modeling.} 
% Masking-based modeling is a machine learning technique, where the fundamental idea is to randomly mask a portion of the input data and then train the model to predict or recover the masked parts. When applying masking-based modeling to graph data, nodes or edges in the graph are typically selected and masked randomly. Subsequently, attempts are made to recover these masked portions based on the remaining graph structural information.
% Because this method emphasizes the recovery of randomly masked parts, it tends to focus more on the details and local structures within the graph. Specifically, it often values small subgraph patterns, the intricate relationships between individual nodes or their neighbors. 
% While the attention to local details ensures the model's high sensitivity in capturing subtle relationships and features within the graph, it might also divert its focus excessively towards these minutiae, potentially overlooking the overarching context and global patterns of the larger graph structures.

\subsection{Definition}


==> sections/2methods.tex <==
\section{Methodology}
\label{sec:meth}

In the framework of \methname shown in Fig.\ref{fig:framework}, we utilize the training objectives of contrastive learning alongside masking-based modeling through a multi-task learning approach. The training pipeline of \methname includes data processing, encoding, and sub-task training.

\subsection{Data Processing}
% 这一段是重点
% 照着GCA重写会是比较好的选择。首先一个preliminary，然后是overall framework。

% 多做几个实验（在TUdataset上），为了让表格填满整个屏幕的宽度。
% 考虑压缩行间距。
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \vspace{-10pt}
  \caption{Experiment results for graph classification. Accuracy(\%) and standard deviation(\%) are reported on all datasets. We highlight the best results in bold for each dataset. The reported results of baselines are from previous papers if available.}
    \vspace{-10pt}
    \begin{tabular}{c|ccc|ccc}
    \hline
    \hline
    Dataset & IMDB-B & IMDB-M & COLLAB & MUTAG & PROTEINS & NCI1 \bigstrut\\
    \hline
    \hline
    WL    & 72.30±3.44 & 46.95±0.46 & -     & 80.72±3.00 & 72.92±0.56 & 80.31±0.46 \bigstrut[t]\\
    DGK   & 66.96±0.56 & 44.55±0.52 & -     & 87.44±2.72 & 73.30±0.82 & 80.31±0.46 \\
    GraphMAE & 75.52±0.66 & 51.63±0.52 & 80.32±0.46 & 88.19±1.26 & \textbf{75.30±0.39} & \textbf{80.40±0.30} \\
    GraphCL & 71.14±0.44 & 48.58±0.67 & 71.36±1.15 & 86.80±1.34 & 74.39±0.45 & 77.87±0.41 \\
    \methname (ours)  & \textbf{75.64±0.25} & \textbf{52.26±1.07} &\textbf{ 82.68±0.74 }& \textbf{89.26±1.56} & 74.72±1.08 & 78.07±0.52 \bigstrut[b]\\
    \hline
    \hline
    \end{tabular}%
    \vspace{-10pt}
  \label{tab:results}%
\end{table*}%

% 这个地方要加多一点的内容，把东西写复杂一点。

The data processing phase of \methname involves graph data augmentation and masking. The objective of data augmentation for graph data is to generate novel and reasonable instances through specific transformation strategies, ensuring that the instance graph maintains semantic similarity to the original graph. In our research, we adopt three data augmentation techniques specifically designed for graph data, including node dropout, edge perturbation, and attribute masking \cite{you2020-graph}. These augmentations are presumed not to alter the inherent semantic label of the graph. 
When a masking-based modeling objective is applied on graph data, one important question is which part of graph should be corrupted and reconstructed. 
Most classical works focus on structure reconstruction \cite{kipf2016variational,pan2018adversarially} where the connectivities between nodes are masked and reconstructed. However, these approaches achieve limited advancement in graph representation learning, which implies that structure provides a global view of how nodes are interrelated. On the other hand, features can provide a local view of what each node represents and what information it carries about its function or role within the network. Thus, we adopt feature masking and reconstruction.
% 可以考虑加一点 mask的比例。

% Formally, let $\mathcal{G}_{i} = \{\mathcal{V}_{i}, \mathcal{E}_{i}, \mathcal{X}_{i}\}$ denote an undirected graph indexed with $i$, where $\mathcal{V}_{i}$ is the node set, $N = |\mathcal{V}_{i} |$ is the number of nodes, $\mathcal{E}_{i}$ is the adjacency matrix, and $\mathcal{X}_{i} \in \mathbb{R}^{N\times d}$ is the input node attribute matrix, then the data processing of $G_{i}$ can be written as:

% \begin{equation}
%     \begin{split}
%         \hat{G_{i}} &= aug(G_{i})\\
%         \tilde{G_{i}} &= mask(G_{i})
%     \end{split}
% \end{equation}

% where $aug(\cdot)$ is data augmentation and $mask(\cdot)$ is graph masking.

% algorithm写复杂一点，多展开一些东西，说明为什么这么做。
\begin{algorithm}[htbp]
	\caption{Training Pipeline of \methname}
	\label{alg:training}
	\textbf{Input:} $\mathcal{G}$: input batch of $N$ graphs where $\mathcal{G}_{i} = \{\mathcal{V}_{i}, \mathcal{E}_{i}, \mathcal{X}_{i}\}$ is the i-th graph in this batch. $\mathbf{M}(\cdot) = \{ \mathbf{E}(\cdot), \mathbf{P}(\cdot), \mathbf{D}(\cdot) \}$ is training model with $\mathbf{E}(\cdot)$ as encoder, $\mathbf{P}(\cdot)$ as projector and $\mathbf{D}(\cdot)$ as decoder.\\
        % \textbf{Output:} Feature Unlearning Model $M_d$
	\begin{algorithmic}[1]
        \FOR{ each $\mathcal{G}_{i}$ in $\mathcal{G}$}
            \STATE $\hat{\mathcal{G}_{i}} \leftarrow AUGMENT(\mathcal{G}_{i})$, $\tilde{\mathcal{G}_{i}} \leftarrow MASK(\mathcal{G}_{i})$
            \STATE $z_{i} \leftarrow \mathbf{P}(\mathbf{E}(\mathcal{G}_{i}))$, $\hat{z_{i}} \leftarrow \mathbf{P}(\mathbf{E}(\hat{\mathcal{G}_{i}})$, $\tilde{z_{i}} \leftarrow \mathbf{P}(\mathbf{E}(\tilde{\mathcal{G}_{i}})$
        \ENDFOR

        \STATE  $\mathcal{L}_{CL} = -\sum^{N}_{i=1}\log \frac{\exp(SIM(z_{i},\hat{z_{i}})/\tau)}{\sum^{N}_{j=1,j\ne i}\exp(SIM(z_{i},\hat{z_{j}})/\tau)}$
        \STATE $\mathcal{L}_{MM}=\frac{1}{N} \sum_{i=1}^{N} (\mathcal{X}_{i} - \mathbf{D}(\tilde{z_{i}}))^2$
        \STATE Determine $\lambda$ based on the training progress.
        \STATE Optimize $\mathbf{M}$ while minimizing $\mathcal{L}=(1-\lambda) \mathcal{L}_{CL} + \lambda \mathcal{L}_{MM}$.
	\end{algorithmic}
        \textbf{Return:} $\mathbf{M}(\cdot)$
\end{algorithm}
\subsection{Encoding}
In the encoding phase, various graph data from previous phase are concurrently fed into both the encoder and projector to obtain embeddings within the projection space. Within our multi-task framework, a singular encoder employed during training which comprises several layers of graph neural networks (GNNs) is shared across distinct tasks. The projector, characterized as a Multi-layer Perceptron (MLP), is tasked with transforming the encoder's output into a dimension more tailored for specific tasks. The backbone for the encoder and the decoder can be any type of GNNs, such as GIN \cite{xu2019-how}, GCN \cite{kipf2016semi} or GAT \cite{velivckovic2018graph}. 
% 补充一点内容。 
% Formulated explicitly, the encoding mechanism is depicted as:

% \begin{equation}
%     z_{i} = MLP(f(\mathcal{G}_{i}))
% \end{equation}

% where \(f(\cdot)\) signifies the multi-layer Graph Neural Network defined.

\subsection{Sub-Task Training}
During the sub-task training, we simultaneously carry out the objectives of globally distinguishing negative sample pairs using contrastive learning and locally reconstructing parts of the masked graph.
For the contrastive learning objective, the aim is to distinguish representations of the original graph and its augmented variant from other negative samples. Embeddings from varied augmentations of the same original graph are pulled closer while those from different graphs are pushed away using normalized temperature-scaled cross entropy loss (NT-Xent) \cite{sohn2016-improved,wu2018-unsupervised,oord2019-representationa}. 
For the masking-based modeling objective, a decoder translates the embeddings from projection space back to the graph space, restoring the masked portions. Given the aim to emphasize the local characteristics of graphs, most node attributes in the graph are masked. After decoding, the mean square error is applied to ensure that the reconstructed graph nodes mirror the original nodes. 
% Here, the normalized temperature-scaled cross entropy loss (NT-Xent) is leveraged to maximize similarity among positive pairs while minimizing it among the negative ones:
% \begin{equation}
%     l_{CL} = -\log \frac{\exp(sim(z_{i},\hat{z_{i}})/\tau)}{\sum^{N}_{j=1,j\ne i}\exp(sim(z_{i},\hat{z_{j}})/\tau)}
% \end{equation}
% where $sim(\cdot)$ denotes the cosine similarity function, with $z_{i}$ and $\hat{z_{i}}$ as the embeddings of $G_{i}$ and $\hat{G_{i}}$ in the projection space, respectively.

% The concluding formula can be written as:

% \begin{equation}
%     l_{masking-based modeling}=mse(\mathcal{G}_{i}.\mathcal{X},decode(\tilde{z_{i}}).\mathcal{X})
% \end{equation}

% where $mse(\cdot)$ denotes mean square error and $decode(\cdot)$ denotes the decoder function.

% The ultimate loss function is a combination of the previously mentioned losses. It can be expressed as:

% \begin{equation}
%      l_{total} = (1-\lambda) l_{CL} + \lambda l_{masking-based modeling} 
% \end{equation}

The pseudocode of training pipeline can be seen in Alg.\ref{alg:training}. The crucial parameter is \( \lambda \), which defines the proportional significance of two distinct loss functions. To harness the unique characteristics of contrastive learning and masking-based modeling across training epochs, we adaptively modulate \( \lambda \) using decrescent dynamic strategy. During the initial training stages, contrastive learning provides a broad global viewpoint. It is desired for the model to first capture this global perspective by assigning a relatively elevated value to \( \lambda \). 
As training progresses and a shift towards emphasizing local features emerges for refinement, \( \lambda \) is progressively decreased, thereby amplifying the masking-based modeling loss. 
This adaptive weighting approach combines the strengths of both learning methods, enabling the model to address local features and global architectures to learn more comprehensive graph representations.

% \subsection{Inference}





==> sections/3experiments.tex <==
\section{Experiments}
\label{sec:exp}
% 分成三个大的实验，就是性能、泛化性、消融
% 泛化性的实验就是简单的说明描述一下，参考graphCL（可以放在性能部分里面）
\subsection{Experimental Settings}

In our experiments, to evaluate \methnametrim's efficacy, we chose comparison methods from both traditional graph kernels and self-supervised learning techniques. Specifically, we considered classic techniques like the Weisfeiler-Lehman subtree kernel (WL) \cite{shervashidze2011weisfeiler} and the Deep Graph Kernel (DGK) \cite{yanardag2015deep}, as well as state-of-the-art methods such as masking-based method GraphMAE \cite{hou2022-graphmae} and contrastive learning method GraphCL \cite{you2020-graph}. 
% These methods represent different developmental stages and learning strategies in graph representation learning.

For the evaluation, we use several benchmark graph datasets from varied domains including bioinformatics datasets like MUTAG, NCI1, and PROTEINS that contain molecular and protein data useful for drug design and socail networks datasets like IMDB-BINARY, IMDB-MULTI, and COLLAB that highlight social network interactions and structures. 
% The statistics of these datasets can be seen in Tab. \ref{tab:dataset}.
% % 这个表放到前面，出现的地方
% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[tb]
%   \centering
%   \caption{Datasets statistics.}
%     \begin{tabular}{c|c|c|c}
%     \hline
%     \hline
%     \multicolumn{1}{l|}{Datasets} & \multicolumn{1}{l|}{Graph Num.} & \multicolumn{1}{l|}{Avg. Nodes} & \multicolumn{1}{l}{Avg. Edges} \bigstrut\\
%     \hline
%     \hline
%     IMDB-B & 1000  & 19.77 & 96.53 \bigstrut[t]\\
%     IMDB-M & 1500  & 13.00 & 65.94 \\
%     % dblp\_ct1 & 755 & 52.87 & 99.78 \\
%     COLLAB & 5000  & 74.49 & 2457.78 \bigstrut[b]\\
%     \hline
%     MUTAG & 188   & 17.93 & 19.79 \bigstrut[t]\\
%     PROTEINS & 1113  & 39.06 & 72.82 \\
%     % AIDS & 2000 & 15.69 & 16.20 \\
%     NCI1  & 4110  & 29.87 & 32.30 \bigstrut[b]\\
%     \hline
%     \hline
%     \end{tabular}%
%   \label{tab:dataset}%
% \end{table}%
\begin{figure*}[tb]
    \centering

    % First image
    \begin{minipage}{0.60\textwidth}  % Adjust width as needed
        \centering
        \begin{adjustbox}{valign=c}
            \includegraphics[width=0.95\linewidth]{image/model_comparison_by_dataset_candid.pdf}
        \end{adjustbox}
        \vspace{-10pt}
        \caption{Ablation experiment results for different components of \methnametrim.}
        \vspace{-13pt}
        \label{fig:model}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.35\textwidth}  % Adjust width as needed
        \centering
        \begin{adjustbox}{valign=c}
            \includegraphics[width=0.95\linewidth]{image/accuracy_comparison_candid.pdf}
        \end{adjustbox}
        \vspace{-5pt}
        \caption{Ablation experiment results for $\lambda$ strategies.}
        \vspace{-13pt}
        \label{fig:lambda}
    \end{minipage}

\end{figure*}

During evaluation, we emphasize \methnametrim's ability to extract deep semantic information from graph data. We follow a generic evaluation method: using \methnametrim's encoder to get graph-level representations, and then feeding these to the LIBSVM classifier \cite{chang2011libsvm}, a renowned SVM classifier. The accuracy and standard deviation from the classifier gave us clear performance metrics. High accuracy indicates effective representation of the original data's key semantics, while the standard deviation shows \methnametrim's consistency across tests. Together, these metrics provide a comprehensive framework for evaluating the generalizability of graph representation models.

\subsection{Performance Comparison and Analysis}


The experimental results are shown in Tab.\ref{tab:results}.
On the social network datasets, \methname  significantly stands out. Specifically, considering the IMDB-B and IMDB-M datasets, it's evident that \methname  surpasses the other methodologies in terms of performance. These datasets often encapsulate intricate structures and multifaceted relationships inherent in social networks. The superior results achieved by \methname  highlight its proficiency in understanding these nuanced connections and the inherent complexities of social network data.
On the bioinformatics datasets, \methname  presents competitive results, though some distinctions should be highlighted. On the NCI1 and PROTEINS datasets, while \methname  performs commendably, it is outperformed by the GraphMAE method. These datasets integrate both comprehensive semantic information and intricate local structural details, crucial in areas like pharmaceutical development and bioinformatics research. Although \methname  shows its ability to process this specialized and complex data, there's evident room for improvement, especially when compared to models like GraphMAE.

% On the bioinformatics datasets, \methname has shown a clear advantage.
% Upon examining the results on the MUTAG, NCI1, and PROTEINS datasets, it is evident that the model excels in grasping the intricacies of biological information. This type of data often integrates rich global semantic information and intricate local structural information, both of which are pivotal in pharmaceutical development and bioinformatics research. The excellent performance of \methname validates its ability to handle this kind of highly specialized and complex data, capturing not just global semantics but also delving into localized structural information.

% As for social network datasets, \methname likewise exhibits robust performance, albeit with some noteworthy distinctions. On the IMDB-B and IMDB-M datasets, \methname leads compared to other methods. This provides us with a valuable observation: varying social network datasets may harbor distinct features and thematic focuses, yet \methname is very close to capturing these complexities in most scenarios. 


\subsection{Ablation Study}
\subsubsection{Diving Deep into Effects of Sub-Tasks}
% 这边放对比没有mae模块和没有gcl模块的消融实验

To understand the effects of the masking-based and contrastive learning objectives on graph representation learning, we evaluated each separately. Specifically, we isolated the two sub-tasks in \methnametrim, creating masking-only and contrastive-only variants. These are then compared on IMDB-B, MUTAG, and PROTEINS.

The results, as depicted in Fig.\ref{fig:model}, show that the complete model consistently outperforms its counterparts on various datasets. This performance stems from its ability to capture both local graph data features and global structural information, indicating a successful integration of the masking-based and contrastive learning strategies.
On IMDB-B and MUTAG datasets, the contrastive-only model outperforms the masking-only variant, highlighting the importance of global graph structures for these tasks. Conversely, on the PROTEINS dataset, the masking model is superior, emphasizing the importance of localized chemical structures in proteins. 

\subsubsection{Adaptive $\lambda$  between Global and Local Balance}
% % 这边放对比使用不同的lambda的消融实验
% Ablation study这里也可以多说一些

% Weights play a pivotal role in balancing contributions from different components of \methname. This experiment delves into the repercussions of static weighting compared to adaptive weighting, aiming to uncover how weight tuning strategies might affect overall model performance. 
% In this study, we explored the following four strategies for the weight \( \lambda \) on IMDB-B and PROTEINS. The decremental dynamic strategy gradually decreases \( \lambda \) from a larger value to a smaller one, while the incremental dynamic strategy does the opposite, increasing \( \lambda \) from a smaller value to a larger one. The masking-focused strategy consistently employes \( \lambda = 0.3 \), and the contrastive-focused strategy utilizes \( \lambda = 0.8 \).

Weights are crucial in balancing \methnametrim's components. We investigated the effects of static versus adaptive weighting, focusing on how different weight tuning strategies influence results. 
We tested four strategies for weight \( \lambda \) on IMDB-B and PROTEINS: the decremental dynamic strategy decreases \( \lambda \) over time, while the incremental dynamic strategy increases it. The masking-focused strategy uses \( \lambda = 0.3 \), and the contrastive-focused strategy sets \( \lambda = 0.8 \).

% Experimental results are shown in \textbf{figure 3}. The results demonstrate significant performance differences among the four strategies on the IMDB-B and PROTEINS datasets. The decremental dynamic strategy starts with a high \( \lambda \), initially leaning towards global feature learning and gradually shifting its focus to local information. In contrast, the incremental Dynamic strategy begins with a lower \( \lambda \), primarily emphasizing local information before transitioning to global features. This might explain its underwhelming performance on IMDB-B, though it excels on the PROTEINS dataset. Comparatively, the masking-focused strategy does not perform well on both datasets. Meanwhile, the contrastive-focused strategy shows improvement over the former, it still trails behind the decremental dynamic strategy, suggesting the superiority of dynamic weight strategies.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.95\linewidth]{image/accuracy_comparison.pdf}
%     \caption{Ablation experiment results for $\lambda$ strategies.}
%     \label{fig:lambda}
% \end{figure}
Shown in Fig.\ref{fig:lambda}, there are notable performance differences among the four strategies on IMDB-B and PROTEINS datasets. 
The decremental dynamic strategy achieves outstanding performance on both datasets, demonstrating the effectiveness of  an early focus on global patterns with shifting attention to local features. The incremental dynamic strategy, on contrast, emphasizes local features before shifting to global ones, resulting in poorer performance on PROTEINS than contrastive-focused one.
Comparatively, the masking-focused strategy does not perform well on both datasets. Meanwhile, the contrastive-focused strategy shows improvement over the former, it still trails behind the decremental dynamic strategy, suggesting the superiority of dynamic weight strategies.

% In conclusion, the decremental dynamic strategy exhibits superior performance on both datasets, confirming its merit in adopting a global-to-local learning paradigm. This method seamlessly integrates the learning of both global and local features and demonstrates remarkable generalizability across varied datasets.

